Detecting Pulsars with Neural Networks: A Proof of Concept

Pulsar searches are computationally demanding efforts to discover dispersed periodic signals in time- and frequency-resolved data from radio telescopes. The complexity and computational expense of simultaneously determining the frequency-dependent delay (dispersion) and the periodicity of the signal is further exacerbated by the presence of various types of radio-frequency interference (RFI) and observing-system effects. New observing systems with wider bandwidths, higher bit rates and greater overall sensitivity (also to RFI) further enhance these challenges. We present a novel approach to the analysis of pulsar search data. Specifically, we present a neural-network-based pipeline that efficiently suppresses a wide range of RFI signals and instrumental instabilities and furthermore corrects for (a priori unknown) interstellar dispersion. After initial training of the network, our analysis can be run in real time on a standard desktop computer with a commonly available, consumer-grade GPU. We complement our neural network with standard algorithms for periodicity searches. In particular with the Fast Fourier Transform (FFT) and the Fast Folding Algorithm (FFA) and demonstrate that with these straightforward extensions, our method is capable of identifying even faint pulsars, while maintaining an extremely low number of false positives. We furthermore apply our analysis to a subset of the PALFA survey and demonstrate that in most cases the automated dispersion removal of our network produces a time series of similar quality as dedispersing using the actual dispersion measure of the pulsar in question. On our test data we are able to make predictions whether a pulsar is present in the data or not 200 times faster than real time.

==> tables/model1_class.tex <==
\begin{table}
\begin{tabular}{cc>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2.5cm}}
\toprule
  # &       JName &  S/N$_{FFA}$ \n Model 1 &  Pulsar Prediction \n Model 1 \\ \hline
\midrule
  1 &  J1957+2831 &                   130.0 &                          1.00 \\
  2 &  J1902+0615 &                    90.2 &                          1.00 \\
  3 &  J1948+2551 &                    69.6 &                          1.00 \\
  4 &  J1850+0026 &                    58.6 &                          1.00 \\
  5 &  J1856+0245 &                    23.7 &                          1.00 \\
  6 &  J1948+2333 &                    30.5 &                          1.00 \\
  7 &  J2005+3547 &                    30.3 &                          1.00 \\
  8 &  J2005+3552 &                    21.8 &                          1.00 \\
  9 &  J2013+3058 &                    16.6 &                          1.00 \\
 10 &  J1850+0423 &                    17.1 &                          1.00 \\
 11 &  J1947+1957 &                    13.9 &                          1.00 \\
 12 &  J1859+0603 &                    11.5 &                          1.00 \\
 13 &  J1858+0346 &                    13.0 &                          0.95 \\
 14 &  J1916+1225 &                     9.6 &                          0.70 \\
 15 &  J1934+2352 &                     9.0 &                          0.01 \\
 16 &  J1855+0307 &                    16.8 &                          1.00 \\
 17 &  J1906+0641 &                    10.5 &                          0.03 \\
 18 &  J2007+3120 &                    10.3 &                          0.61 \\
 19 &  J1902+0615 &                    11.0 &                          0.49 \\
 20 &  J1848+0351 &                    10.2 &                          0.02 \\
 21 &  J1906+0641 &                    11.4 &                          1.00 \\
 22 &  J1851+0418 &                     7.1 &                          0.03 \\
 23 &  J1946+2535 &                     7.6 &                          0.06 \\
 24 &  J1908+0909 &                     5.8 &                          0.26 \\
\bottomrule
\end{tabular}
\label{tab:model1_class}
\caption{Comparison between the FFA S/N and the classification result of Model 1. The pulsar prediction is the median of the cross validation runs.}
\end{table}

==> tables/psr_table.tex <==
\begin{table*}
\begin{tabular}{cc>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2cm}}
%\toprule
  # &        PSR \newline JName &  DM \newline (pc cm$^{-3}$) &  Period \newline (ms) &  S/N$_{FFA}$ \n Dedispersion &  S/N$_{FFA}$ \n Model 1 &  S/N$_{FFA}$ \n Model 2 &  S/N$_{FFA}$ \n Model 3 \\ \hline
%\midrule
  1 &  J1957+2831 &                         138 &                   307 &                         94.1 &                   130.0 &                   130.7 &                   137.5 \\
  2 &  J1902+0615 &                         502 &                   673 &                         59.1 &                    90.2 &                    91.1 &                   107.7 \\
  3 &  J1948+2551 &                         289 &                   196 &                         50.7 &                    69.6 &                    71.7 &                    79.0 \\
  4 &  J1850+0026 &                         201 &                  1081 &                         47.0 &                    58.6 &                    49.2 &                    64.9 \\
  5 &  J1856+0245 &                         623 &                    80 &                         20.4 &                    23.7 &                     8.0 &                    19.1 \\
  6 &  J1948+2333 &                         198 &                   528 &                         17.9 &                    30.5 &                    26.9 &                    26.5 \\
  7 &  J2005+3547 &                         401 &                   615 &                         16.8 &                    30.3 &                    31.3 &                    47.9 \\
  8 &  J2005+3552 &                         455 &                   307 &                         14.7 &                    21.8 &                    18.0 &                    22.7 \\
  9 &  J2013+3058 &                         148 &                   276 &                         12.3 &                    16.6 &                    14.5 &                    10.3 \\
 10 &  J1850+0423 &                         265 &                   290 &                         11.9 &                    17.1 &                    16.8 &                    15.2 \\
 11 &  J1947+1957 &                         185 &                   157 &                          9.8 &                    13.9 &                    13.1 &                     8.1 \\
 12 &  J1859+0603 &                         378 &                   508 &                          8.9 &                    11.5 &                    12.4 &                     8.4 \\
 13 &  J1858+0346 &                         386 &                   256 &                          8.8 &                    13.0 &                    12.8 &                    10.8 \\
 14 &  J1916+1225 &                         265 &                   227 &                          8.8 &                     9.6 &                     9.6 &                     9.5 \\
 15 &  J1934+2352 &                         355 &                   178 &                          7.9 &                     9.0 &                     9.3 &                     9.1 \\
 16 &  J1855+0307 &                         402 &                   845 &                          7.8 &                    16.8 &                    14.1 &                    17.4 \\
 17 &  J1906+0641 &                         472 &                   267 &                          7.6 &                    10.5 &                     8.4 &                     8.2 \\
 18 &  J2007+3120 &                         191 &                   608 &                          7.4 &                    10.3 &                     9.1 &                     7.7 \\
 19 &  J1902+0615 &                         502 &                   673 &                          6.9 &                    11.0 &                     8.9 &                    11.3 \\
 20 &  J1848+0351 &                         336 &                   191 &                          6.9 &                    10.2 &                    10.1 &                     6.1 \\
 21 &  J1906+0641 &                         472 &                   267 &                          6.6 &                    11.4 &                     8.5 &                     8.7 \\
 22 &  J1851+0418 &                         115 &                   284 &                          6.1 &                     7.1 &                     6.3 &                     5.5 \\
 23 &  J1946+2535 &                         248 &                   515 &                          5.1 &                     7.6 &                     6.7 &                     6.6 \\
 24 &  J1908+0909 &                         467 &                   336 &                          3.4 &                     5.8 &                     4.9 &                     6.6 \\
%\bottomrule
\end{tabular}




\label{tab:psr}
\caption{Pulsars that are observable in the test data set and their period and DM. Also shown is the S/N of the pulsar signal in the FFA of both the dedispersed output and the intermediate output of the various neural network models. The dedispersed output was downsampled by a factor of 4 after dedispersing to make a better comparison possible. In models with multiple output channels the higher S/N is given.}
\end{table*}


==> tables/psr_table_pred_single.tex <==
\begin{landscape}
\begin{table}
\begin{tabular}{cc>{\raggedleft\arraybackslash}p{1.8cm}>{\raggedleft\arraybackslash}p{1.8cm}>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{2cm}>{\raggedleft\arraybackslash}p{1.8cm}>{\raggedleft\arraybackslash}p{1.8cm}>{\raggedleft\arraybackslash}p{1.8cm}}
%\toprule
    &       JName &  \centering DM \newline (pc cm$^{-3}$) & \centering Period \newline (ms) &  \centering S/N$_{FFA}$ \newline Dedispersion &  \centering N$_{FFA}$ \newline Model 1 & \centering S/N$_{FFA}$ \newline Model 2 & \centering S/N$_{FFA}$ \newline Model 3 &  \centering Prediction \newline Model 1 & \centering Prediction \newline Model 2 & \centering Prediction \newline Model 3 \cr\\ \hline
%\midrule
  1 &  J1902+0615 &                                  502 &                            673 &                                        110.9 &                                  133.0 &                                  139.2 &                                  152.7 &                                  1.00 &                                  1.00 &                                  1.00 \\
  2 &  J1957+2831 &                                  138 &                            307 &                                         74.8 &                                  135.2 &                                  126.2 &                                  146.6 &                                  1.00 &                                  1.00 &                                  1.00 \\
  3 &  J1850+0026 &                                  201 &                           1081 &                                         53.3 &                                   92.5 &                                   83.0 &                                   98.1 &                                  1.00 &                                  1.00 &                                  1.00 \\
  4 &  J1948+2551 &                                  289 &                            196 &                                         53.0 &                                   67.3 &                                   65.6 &                                   82.0 &                                  1.00 &                                  1.00 &                                  1.00 \\
  5 &  J1948+2333 &                                  198 &                            528 &                                         35.3 &                                   43.1 &                                   36.3 &                                   46.2 &                                  1.00 &                                  1.00 &                                  1.00 \\
  6 &  J2005+3547 &                                  401 &                            615 &                                         25.8 &                                   34.7 &                                   31.5 &                                   52.3 &                                  1.00 &                                  1.00 &                                  1.00 \\
  7 &  J1856+0245 &                                  623 &                             80 &                                         21.4 &                                   16.0 &                                    5.1 &                                    6.5 &                                  1.00 &                                  0.09 &                                  0.94 \\
  8 &  J2005+3552 &                                  455 &                            307 &                                         15.7 &                                   20.0 &                                   15.1 &                                   15.1 &                                  1.00 &                                  1.00 &                                  1.00 \\
  9 &  J1855+0307 &                                  402 &                            845 &                                         15.5 &                                   19.1 &                                   16.7 &                                    5.6 &                                  1.00 &                                  1.00 &                                  0.06 \\
 10 &  J2013+3058 &                                  148 &                            276 &                                         14.0 &                                   15.7 &                                   13.5 &                                    5.3 &                                  1.00 &                                  1.00 &                                  0.11 \\
 11 &  J1947+1957 &                                  185 &                            157 &                                         13.4 &                                   13.8 &                                   12.2 &                                    5.3 &                                  1.00 &                                  1.00 &                                  0.10 \\
 12 &  J1902+0615 &                                  502 &                            673 &                                         11.4 &                                   12.7 &                                    7.7 &                                    1.1 &                                  1.00 &                                  0.64 &                                  0.96 \\
 13 &  J1850+0423 &                                  265 &                            290 &                                         11.4 &                                   16.1 &                                   14.7 &                                    5.8 &                                  1.00 &                                  1.00 &                                  0.10 \\
 14 &  J1934+2352 &                                  355 &                            178 &                                         11.2 &                                    7.8 &                                    8.1 &                                    5.1 &                                  0.46 &                                  0.88 &                                  0.07 \\
 15 &  J1916+1225 &                                  265 &                            227 &                                         10.1 &                                    8.8 &                                    8.4 &                                    4.9 &                                  1.00 &                                  0.99 &                                  0.17 \\
 16 &  J1906+0641 &                                  472 &                            267 &                                          9.8 &                                   11.6 &                                    9.4 &                                    5.5 &                                  1.00 &                                  1.00 &                                  0.08 \\
 17 &  J1859+0603 &                                  378 &                            508 &                                          9.8 &                                   12.4 &                                   13.0 &                                    7.1 &                                  1.00 &                                  1.00 &                                  0.36 \\
 18 &  J2007+3120 &                                  191 &                            608 &                                          9.4 &                                   12.7 &                                    9.3 &                                    4.4 &                                  1.00 &                                  1.00 &                                  0.06 \\
 19 &  J1946+2535 &                                  248 &                            515 &                                          9.3 &                                    9.4 &                                    9.0 &                                    4.4 &                                  0.97 &                                  0.99 &                                  0.08 \\
 20 &  J1848+0351 &                                  336 &                            191 &                                          9.1 &                                    8.0 &                                    8.3 &                                    5.1 &                                  0.76 &                                  0.96 &                                  0.18 \\
 21 &  J1906+0641 &                                  472 &                            267 &                                          8.7 &                                    9.6 &                                    6.5 &                                    4.3 &                                  1.00 &                                  0.21 &                                  0.08 \\
 22 &  J1858+0346 &                                  386 &                            256 &                                          8.0 &                                   10.9 &                                   10.8 &                                    5.9 &                                  1.00 &                                  1.00 &                                  0.08 \\
 23 &  J1908+0909 &                                  467 &                            336 &                                          5.4 &                                    4.5 &                                    4.1 &                                    3.4 &                                  0.08 &                                  0.06 &                                  0.07 \\
 24 &  J1851+0418 &                                  115 &                            284 &                                          5.3 &                                    6.1 &                                    5.2 &                                    4.7 &                                  0.05 &                                  0.06 &                                  0.10 \\
%\bottomrule
\end{tabular}
\label{tab:psr}
\caption{Pulsars in the test set and their S/N in the FFA of the dedispersed output and the output of the neural networks. When the network has multiple output channels the stronger signal was used. Also shown is the pulsar prediction of the networks. Since for each model five networks where trained the median is shown for both the S/N and the pulsar prediction. The dedispersed output was created after removing the mean of each time step and was downsampled by a factor of 4 after dedispersing.}
\end{table}
\end{landscape}
